Inferring the Long-Term Causal Effects of Long-Term Treatments from Short-Term Experiments

We study inference on the long-term causal effect of a continual exposure to a novel intervention, which we term a long-term treatment, based on an experiment involving only short-term observations. Key examples include the long-term health effects of regularly-taken medicine or of environmental hazards and the long-term effects on users of changes to an online platform. This stands in contrast to short-term treatments or "shocks," whose long-term effect can reasonably be mediated by short-term observations, enabling the use of surrogate methods. Long-term treatments by definition have direct effects on long-term outcomes via continual exposure, so surrogacy conditions cannot reasonably hold. We connect the problem with offline reinforcement learning, leveraging doubly-robust estimators to estimate long-term causal effects for long-term treatments and construct confidence intervals.

==> old_experiments.tex <==
To demonstrate the effectiveness of the ORL method, we perform experiments on simulated data. In particular, we compare the method against a baseline surrogate index method in estimating a range of known long-term ATEs, each associated with a different treatment duration regime. Code and data for the experiments is available at: \url{https://github.com/allentran/long-term-ate-orl}. 

The results confirm that the surrogate index method recovers the true long-term ATE, albeit only for a treatment of duration of a single period. When applied to data from experiments with treatment durations longer than a single period, the estimate remains static and hence its bias grows with the underlying treatment duration. On the other hand, the ORL method produces estimates that match the true ATE, growing as the duration of treatment extends from a single period to permanent.

\subsection{Simulation Details}
We generate ground truth data for the experiments with features that mirror those typically found within personalization algorithm tests for a global streaming video on demand service. In particular, we construct a single state Markov chain that mimics the dynamics of on-service tenure. Over time, on-service tenure increases if members do not churn, which we model as a drift-diffusion process with positive drift:
\begin{equation}
    s_t = s_{t-1} + \mu + \sigma_s w_t
    \label{eq:sim_states}
\end{equation}
where $w_t \sim \mathcal{N}(0, 1)$ and we restrict $s_t \in [0, 1]$ by clipping.

To reflect that longer tenured members often have higher per period revenue, we set the reward to be a diminishing scalar multiple of the state.
\begin{equation}
    y_t = \alpha s_t^\theta + \sigma_r e_t
    \label{eq:sim_reward}
\end{equation}
where $e_t \sim \mathcal{N}(0, 1)$.

We assume that treatment effects both increase the probability of a transition to a higher state and increase average per-period rewards conditional on the state. These are implemented as positive constants in Equations \eqref{eq:sim_states} and \eqref{eq:sim_reward} when the treatment is active in that period. This mirrors the decomposition of long term treatment effects in Equation \eqref{eq:decomp_ate}. Table \ref{tab:freq} lists the parameter values used in the experiments. For simplicity, we assume the experiment lasts a single period, with all variables observed in the first period as well as the transition to the second period state.

\begin{table}
  \caption{Simulation Parameter Values}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Notation&Description&Value\\
    \midrule
    $\gamma$ & Discount rate & 0.9 \\
    $\mu$ & Drift in state transition& 0.05\\
    $\sigma_s$ & Std. dev. in state transition in 5& 0.1\\
    $\sigma_r$ & Std. dev. in state-outcome mapping & 0.1\\
    $\theta $ & Curvature in state-outcome mapping & 0.8\\
    $\tau_s$ & Treatment effect on state transition& 0.05\\
    $\tau_y$ & Treatment effect on per-period outcome& 0.01\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Model Implementation Details}
The baseline surrogate index method estimates the potential outcome means for the first period as empirical means for each of treatment and control. To project long term outcomes, we first construct a synthetic long term observational dataset by simulating trajectories over a long horizon where treatment effects are set to zero. We then fit a regression model using the Random Forests algorithm where the input features is just the surrogate, the state from the second period, and the target is the normalized discounted sum of outcomes from the second period onwards.\footnote{We use the defaults from the scikit-learn package. Although we could tune hyperparameters, the estimates using the defaults match the single period treatment ATE almost perfectly.} The long-term estimand is obtained by combining the two by adding the first period potential outcome means to the discounted sum of outcomes from the second period onwards, discounted and normalized appropriately.

To demonstrate the effectiveness of the surrogate index method when its assumptions hold, we estimate a variant where the surrogacy assumption holds even with a long treatment: the surrogate mediates the long-term treatment effect. To do, we must include data from the experiment up to the last treatment period. In doing so, we effectively create a intermediate-term experiment, which moves us away from the central constraint of the paper, that of a \textit{short} experiment.\footnote{Note that the intermediate-term experiment is not the same as observing the entire experiment since the surrogate method only sees data up to the last treatment period.}

The ORL method requires the estimation of two nuisance functions, the $Q$ function and the density ratio functions. For the $Q$ function, we use a feed-forward neural network parameterized separately for each of treatment and control. Each network consists of a single hidden layer with 48 features and a sigmoid activation function and a linear final layer with no activation function. Additionally, we maintain separate ``target'' networks by freezing the parameters of each network for 32 epochs, which proved invaluable in stabilizing training \cite{mnih2015humanlevel}.

For the density ratio functions, we use the Minimax weight estimator from \citet{ueharaminimax} where we restrict both the discriminator and density ratio function classes to be linear with the feature maps $\phi(s) = \begin{bmatrix} s & s^2 & 1 \end{bmatrix}$.

\subsection{Results}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{qw.experiments.png} % Replace "filename" with your image file's name, without the extension
    \caption{Estimates of the ATE for differing treatment durations}
    \label{fig:experiments}
\end{figure}

Figure \ref{fig:experiments} shows the results of simulations of A/B tests where the treatment arm has treatment active for the first 1, 6, 12, 24, 48 and $\infty$ periods and no treatment thereafter. From the entire history of the each experiment, we calculate the true long-term ATE. In contrast, to mimic real-world scenarios, the estimators evaluated only see a fraction of the underlying data from the experiment.

Since the treatment increases both the state-outcome mapping and the likelihood of a positive state transition, the true ATE (red) increases with the duration of the treatment. Estimates from the ORL method (blue) match the true ATE, as the duration of treatment extends all the way to a permanent intervention. 

As Section \ref{sec:surrogate_comp} previewed, the surrogate index method estimates long term outcomes as if treatment is applied up to the point at which the last surrogate is measured regardless of the underlying treatment duration. Hence the baseline method (green), where the surrogate is the second period state, estimates the long-term ATE for when treatment is active only for a single period. The estimate is constant and therefore underestimates the true ATE for $T>1$.

On the other hand, if one is explicit about the treatment duration of interest and measures surrogates up to that point, the intermediate-term surrogate method (purple) matches the true ATE. While both methods match the true ATE, their requirements on measurement are vastly different. The key benefit of the ORL method is that one can estimate the long term ATE from an arbitrary duration treatment regime with a short experiment. With the ORL method, the requirements on the duration of measurement remain static independent of the treatment duration of interest. However, one downside is that the variance of the ORL estimates appear to be larger than the surrogate methods. 

